Isoperimetric sets in nonnegative scalar curvature and their role through various concepts of mass

We review some recent results about the relations among isoperimetric sets, Penrose inequalities and related concepts in the analysis of $3$-manifolds of nonnegative scalar curvature. We also show that if the isoperimetric sets of big volume have connected boundaries, the equivalence among suitable notions of mass hold.

==> introduzione.tex <==
The concept of ADM mass, introduced in the early sixties by the physicists Arnowitt, Deser and Misner \cite{arnowitt_coordinate_1961}, plays a central role in the modern development of mathematical relativity, because of both its physical relevance and its intriguing geometric features. On
the initial datum of a given isolated gravitational system, modelled by 
an Asymptotically Flat $3$-manifold $(M,g)$ with nonnegative scalar curvature, the $\ADM$ mass is given by
\begin{equation}\label{eq:mADM}
 \ma_{\ADM} = \lim_{j \to +\infty}\frac{1}{16\pi} \int_{\partial\Omega_j}g^{ij}(\partial_k g_{ij}- \partial_i g_{kj} ) \nu^k \dif \sigma \, ,
\end{equation}
where the flux integrals are taken along the boundaries of some exhaustion $(\Omega_j)_{j \in \N}$ of $M$, $\nu$ and $\dd \sigma$ being the unit normal vector field and the volume measure on $\partial \Omega_j$, respectively.  In the above formula, the metric coefficients, as well as their partial derivatives, are expressed in a given \emph{asymptotically flat coordinate chart} $(x^1,x^2,x^3)$ (see \cref{def:asyflat}). Therefore, the value of the $\ADM$ mass is a priori coordinates dependent. However, in a couple of remarkable papers \cite{bartnik_mass_1986, chrusciel_boundary_1986}, it has been shown that the above expression defines a geometric invariant, provided the metric $g$ is $\CS^{1}_\tau$--Asymptotically Flat, with $\tau > 1/2$. This means that $\abs{x}^\tau\abs{g_{ij}-\delta_{ij}} = O_1(1)$ at infinity. In such a context, $\ma_{\ADM}$ is finite if and only if the scalar curvature is integrable on the whole space.

The most important statement about the $\ADM$ mass is the so called Positive Mass Theorem, firstly proven by Schoen and Yau \cite{schoen_proof_1979, schoen_proof_1981} and subsequently by Witten \cite{witten_new_1981,parker_witten_1982}. It says that $\ma_{\ADM}$ is nonnegative, and it is equal to zero if and only if $(M,g)$ is isometric to the flat Euclidean space. 

A sharper lower bound for the $\ADM$ mass was conjectured by Penrose \cite{penrose_naked_1973} for Asymptotically Flat $3$-manifolds with nonnegative scalar curvature containing a horizon boundary $N$, which are known to model initial data sets of space-times containing a black-hole. It says that in this case the $\ADM$ mass cannot be smaller than the square root of the area of the horizon, normalized by a suitable dimensional constant.
\begin{equation}
\sqrt{\frac{ \abs{ N}}{16 \pi}} \leq \ma_{\ADM},
\end{equation}
where equality is achieved on the standard space-like slice of a Schwarzschild space-time. Loosely speaking, the total mass of an Asymptotically Flat solution containing a black-hole must be at least as large as the total mass of a Schwarzschild solution, having the same horizon's area. 

Such a remarkable statement, known as the Riemannian Penrose Inequality, was first proven by Huisken and Ilmanen \cite{huisken_inverse_2001}, in the case of connected horizon, using the weak Inverse Mean Curvature Flow (IMCF for short). Concurrently, Bray \cite{bray_proof_2001} was able to prove the same statement in the case of multiple black-holes, establishing a monotonicity formula for the $\ADM$ mass along a suitably constructed conformal flow of metrics. Bray's proof was subsequently extended up to dimension $7$, by Bray and Lee \cite{bray_riemannian_2009}. Very recently, a new proof of the single black-hole statement has been proposed by the third author, in a joint work with Agostiniani, Mantegazza and Oronzio \cite{agostiniani_riemannian_2022}, using the level sets flow of $p$-harmonic functions. 

A common feature of the above mentioned results is the fact that the requirements on the asymptotic behaviour of the metric are not optimal, in that the decay rate which is needed to establish the inequality is stronger than the one that is needed to define the mass. More precisely, in Huisken-Ilmanen's proof through weak IMCF, and similarly in the one through $p$-harmonic potentials \cite{agostiniani_riemannian_2022}, the metric $g$ is assumed to be $\CS^1_1$--Asymptotically Flat. Moreover, the Ricci tensor is required to obey the following quadratic decay condition $\Ric \geq - \kst\abs{x}^{-2} g$, where $(x^1,x^2,x^3)$ are asymptotically flat coordinates and $C>0$ is a given constant.
On the other hand, Bray's version of the Penrose Inequality \cite{bray_proof_2001}, holding also in the presence of possibly disconnected horizons, is proved requiring $\CS^{2}_\tau$--asymptotic flatness, for some $\tau>1/2$. 

Asymptotic conditions on the second derivatives of the metric coefficients are in fact commonly assumed even in the proof of the Positive Mass Theorem, as it can be checked following either the classical arguments by Schoen and Yau \cite{schoen_proof_1979, schoen_proof_1981} and Witten \cite{witten_new_1981,parker_witten_1982}, or through some recent alternative proofs, as the ones proposed in \cite{bray_harmonic_2022} and in \cite{agostiniani_green_2021}. In particular, to the best of our knowledge, not even the Positive Mass Theorem is known to hold under the optimal decay assumptions yet. Our first main result fills this gap,  establishing the validity of the single horizon Riemannian Penrose Inequality, under the sole decay assumptions that make the $\ADM$ mass a well defined geometric invariant. 

\begin{theorem}[Riemannian Penrose Inequality under optimal decay assumptions]
\label{thm:penrose_adm_intro}
Let $(M,g)$ be a complete $\CS^{1}_{\tau}$-Asymptotically Flat Riemannian $3$-manifold, $\tau >1/2$, with nonnegative scalar curvature and smooth, compact, minimal and outward minimising (possibly empty) boundary. Assume that $H_2( M, \partial M; \Z)=\set{0}$. Then, it holds
\begin{equation}\label{eq:adm_penrose}
 \sqrt{\frac{ \abs{N}}{16 \pi}} \leq \ma_{\ADM},
\end{equation}
where $N$ is any connected component of $\partial M$, with the equality satisfied if and only if $\partial M$ is connected and $(M,g)$ is isometric to a space-like slice of the Schwarzschild manifold
\begin{equation}
 \left(\R^n\smallsetminus \set{ \abs{x} < 2 \ma_{\ADM}} \, , \left( \! 1+ \frac{ \ma_{\ADM}}{2 \abs{x}} \!\right)^{\!\!4}\eum_{ij} \,\, \dd x^i \! \otimes \dd x^j\right).
\end{equation}
\end{theorem}
Some comments are in order. As observed in \cite[Lemma 4.1]{huisken_inverse_2001}, the topological assumption $H_2( M, \partial M; \Z)=\set{0}$ is automatically satisfied if $M$ is an \emph{exterior region}, i.e., it is connected and asymptotically flat, has a compact, minimal boundary, and contains no other compact minimal surfaces (even immersed). Technically, the vanishing of the second relative homology group guarantees that the weak IMCF of a connected hypersurface remains connected for all times. This fact is crucial in the Huisken-Ilmanen approach, as it allows to invoke the Gauss-Bonnet Theorem in the computations leading to Geroch Monotonicity Formula. 



The statement of \cref{thm:penrose_adm_intro} holds true even when $\partial M = \varnothing$, where it gives the Positive Mass Theorem under optimal decay assumptions. In this case, the topological assumption becomes $H_2( M; \Z)=\set{0}$, and the rigidity statement is phrased in terms of the flat $3$-dimensional Euclidean space, which is understood as a zero-mass Schwarzschild space.

\medskip

Along the route to \cref{thm:penrose_adm_intro} we establish a Riemannian Penrose Inequality for the \emph{Isoperimetric mass}, which constitutes in fact our second main result. This pretty general and very geometric concept of mass was introduced by Huisken in \cite{huisken_isoperimetric_2006}. Hereafter, we recall its definition.

\begin{definition}[Isoperimetric mass] \label{def:isoperimetric_mass}
Let $(M,g)$ be a noncompact Riemannian $3$-manifold and let $\Omega$ be a closed bounded subset $\Omega\subset M$ with $\CS^{1,\alpha}$--boundary. The quasi-local Isoperimetric mass of $\Omega$ is defined as
\begin{equation}\label{eq:quasi-local_isoperimetric_mass_intro}
 \ma_{\iso}(\Omega)=\frac{2}{\abs{\partial \Omega}}\left( \abs{\Omega} -\frac{\abs{\partial \Omega}^{\frac{3}{2}}}{6 \sqrt{\pi}}\right).
\end{equation}
The Isoperimetric mass $\ma_{\iso}$ of $(M,g)$ is then defined as \begin{equation}\label{eq:isoperimetric_mass_intro}
 \ma_{\iso}=\sup_{(\Omega_j)_{j\in \N}}\limsup_{j \to +\infty} \ma_{\iso}(\Omega_j),
\end{equation}
where the supremum is taken among all exhaustions $(\Omega_j)_{j\in \N}$ consisting of domains with $\CS^{1,\alpha}$--boundary. 
\end{definition}

It is immediately clear that the Isoperimetric mass does not require any particular assumption on the asymptotic character of the metric in order to be well defined. Hence, the question arises whether a Riemannian Penrose inequality is available for such a mass and for a broader class of initial data sets. A first answer to this question can be found in \cite{jauregui_lower_2021}, where the authors, following and strengthening the original argument of Huisken \cite{huisken_isoperimetric_2006}, are able to prove that the Isoperimetric mass coincides with the $\ADM$ mass if the metric is assumed to be $\CS^2_\tau$--Asymptotically Flat at infinity. An alternative proof in the same setting has been worked out in \cite[Appendix C]{chodosh_isoperimetry_2021}.

In the present paper, we extend the Isoperimetric Riemannian Penrose Inequality to the class of {\em strongly $1$-nonparabolic spaces}. This locution, which is inspired by the notion of {\em strongly nonparabolic spaces} introduced in \cite{ni_mean_2007}, indicates Riemannian manifolds $(M,g)$ such that, for every $\Omega\subset M$  with smooth boundary homologous to $\partial M$, there exists a proper solution $w_1\in \Lip_{\loc}(M\smallsetminus \Int \Omega)$ to the weak IMCF problem starting at $\partial \Omega$
\begin{equation}\label{eq:IMCF}
 \begin{cases}
 \div\left( \dfrac{ \D w_1}{\abs{\D w_1}}\right) &=& \abs{ \D w_1} & \text{on $M\smallsetminus \Omega$,}\\
 w_1 &=& 0 & \text{on $\partial \Omega$,}\\
 w_1 &\to& +\infty & \text{as $\dist(x,o) \to +\infty$}.
 \end{cases}
\end{equation} 
We can now state our second main result.

\begin{theorem}[Isoperimetric Riemannian Penrose Inequality]
\label{thm:isoperimetric_penrose_intro}
Let $(M,g)$ be a complete strongly $1$-nonparabolic Riemannian $3$-manifold, with nonnegative scalar curvature and smooth, compact, minimal and outward minimising (possibly empty) boundary. Assume that $H_2( M, \partial M; \Z)=\set{0}$. Then, it holds
\begin{equation}\label{eq:isoperimetric_penrose}
 \sqrt{\frac{ \abs{N}}{16 \pi}} \leq \ma_{\iso},
\end{equation}
where $N$ is any connected component of $\partial M$, with the equality satisfied if and only if $\partial M$ is connected and $(M,g)$ is isometric to a space-like slice of the Schwarzschild manifold
\begin{equation}
 \left(\R^n\smallsetminus \set{ \abs{x} < 2 \ma_{\iso}} \, , \left( \! 1+ \frac{ \ma_{\iso}}{2 \abs{x}} \!\right)^{\!\!4}\eum_{ij} \,\, \dd x^i \! \otimes \dd x^j\right).
\end{equation}
\end{theorem}
 We notice once more that the above result does not require any specific decay of the metric coefficients towards the Euclidean model. The strong $1$-nonparabolicity condition is satisfied for example on manifolds with lower Ricci bounds and such that an Euclidean-like Isoperimetric inequality holds \cite[Theorem 1.7]{mari_flow_2022}, or whenever there exists a subsolution to \cref{eq:IMCF} starting at some bounded subset \cite[Weak Existence Theorem 3.1]{huisken_inverse_2001}.
Finally, we realise that in the setting of \cref{thm:penrose_adm_intro} the isoperimetric mass actually coincides with the $\ADM$ mass (see \cref{thm:mass_equivalence}), improving \cite[Theorem 3]{jauregui_lower_2019}. 

\medskip

\cref{thm:isoperimetric_penrose_intro} provides new information also in the basic situation of manifolds that are $\CS^0$--asymptotic to a Schwarzschild space of nonnegative mass $\ma$ (see \cref{def:asysvar}). Indeed, in \cref{thm:asysvarchild} below, we show that such parameter satisfies the expected Penrose Inequality and that it coincides in fact with the Isoperimetric mass. We emphasise that in this setting the classical notion of $\ADM$ mass is not even clearly defined, as it involves the asymptotic behaviour of derivatives of the metric coefficients.

\begin{theorem}[Penrose Inequality in Asymptotically Schwarzschildian manifolds]
\label{thm:asysvarchild}
Let $(M, g)$ be a $\CS^0_\tau$-Asymptotically Schwarzschildian Riemannian $3$-manifold of mass $\ma \geq 0$, $\tau>0$, with nonnegative scalar curvature and smooth, compact, minimal and outward minimising (possibly empty) boundary. Assume that $H_2(M, \partial M; \Z) = \set{0}$. Then, it holds
 \begin{equation}
 \label{eq:penrose-svarchild}
 \sqrt{\frac{\abs{N}}{16 \pi}}\leq \ma,
\end{equation}
where $N$ is any connected component of $\partial M$, with the equality satisfied if and only if $\partial M$ is connected and $(M,g)$ is isometric to a space-like slice of the Schwarzschild manifold
\begin{equation}
 \left(\R^n\smallsetminus \set{ \abs{x} < 2 \ma} \, , \left( \! 1+ \frac{ \ma}{2 \abs{x}} \!\right)^{\!\!4}\eum_{ij} \,\, \dd x^i \! \otimes \dd x^j\right).
\end{equation}
Moreover, we have
\begin{equation}
\label{eq:identity-massiso} 
\ma = \ma_{\iso}. 
\end{equation}
\end{theorem}












% \bigskip
% \bigskip
% \bigskip

% \bigskip
% \bigskip
% \bigskip


% The $\ADM$ mass of an Asymptotically Flat $3$-manifold $(M,g)$ with nonnegative scalar curvature has been introduced by \cite{arnowitt_coordinate_1961} as a geometric invariant that represents the total mass of a time-symmetric initial data set for Einstein's equations. This quantity is given by a flux integral through the boundary of some exhaustion $(\Omega_j)_{j \in \N}$ of the space, namely
% \begin{equation}\label{eq:mADM}
%  \ma_{\ADM} = \lim_{j \to +\infty}\frac{1}{16\pi} \int_{\partial\Omega_j}g^{ij}(\partial_k g_{ij}- \partial_i g_{kj} ) \nu^k \dif \sigma
% \end{equation}
% where $\nu$ and $\dd \sigma$ are the $g$-unit normal vector field and the volume measure on $\partial \Omega_j$. All quantities are expressed with respect to an \emph{asymptotically flat coordinate chart}. This concept of mass is well known to be well-defined if the metric is $\CS^{1}_\tau$- Asymptotically Flat with $\tau > 1/2$ (\cite{bartnik_mass_1986, chrusciel_boundary_1986}). With this notation we are substantially indicating a metric $g$ such that $\abs{x}^\tau\abs{g-\delta} = O_1(1)$ at infinity, see \cref{def:asyflat}. Moreover, it is finite exactly when the scalar curvature is integrable on the whole space.


% \smallskip

% As desirable by any concept of mass, Schoen and Yau \cite{schoen_proof_1979, schoen_proof_1981} and Witten \cite{witten_1981} proved that this quantity is nonnegative, equaling zero only in the flat Euclidean case. 

% A stronger result, first conjectured by Penrose, holds on Asymptotically Flat $3$-manifolds with nonnegative scalar curvature with horizon boundary $N$. It reads
% % The Riemannian version of a famous conjecture by Penrose \cite{penrose_naked_1973} reads as
% \begin{equation}
% \sqrt{\frac{ \abs{ N}}{16 \pi}} \leq \ma_{\ADM},
% \end{equation}
% and is known as Riemannian Penrose Inequality.
% This striking result has been proved for connected horizons by Huisken and Ilmanen \cite{huisken_inverse_2001} using the weak Inverse Mean Curvature Flow (IMCF for short) and Bray \cite{bray_proof_2001} using Monotonicity Formulas for the $\ma_{\ADM}$ along a flow of conformal metrics. The latter method actually works also for disconnected boundaries. Very recently, a new proof based on Nonlinear Potential Theory has been proposed by the third author together with Agostiniani, Mantegazza and Oronzio \cite{agostiniani_riemannian_2022}.


% \bigskip
% \bigskip
% \bigskip





% In recent years, many concepts of mass have been introduced, in addition to the $\ma_{\ADM}$. We recall Huisken's Isoperimetric mass \cite{huisken_isoperimetric_2006}, a main object of the present work.

% \begin{definition}[Isoperimetric mass] \label{def:isoperimetric_mass}
% Let $(M,g)$ be a noncompact Riemannian $3$-manifold. Given a closed bounded subset $\Omega\subset M$ with $\CS^{1,\alpha}$-boundary the quasi-local Isoperimetric mass of $\Omega$ is defined as
% \begin{equation}\label{eq:quasi-local_isoperimetric_mass_intro}
%  \ma_{\iso}(\Omega)=\frac{2}{\abs{\partial \Omega}}\left( \abs{\Omega} -\frac{\abs{\partial \Omega}^{\frac{3}{2}}}{6 \sqrt{\pi}}\right).
% \end{equation}
% The Isoperimetric mass $\ma_{\iso}$ of $(M,g)$ is defined as \begin{equation}\label{eq:isoperimetric_mass_intro}
%  \ma_{\iso}=\sup_{(\Omega_j)_{j\in \N}}\limsup_{j \to +\infty} \ma_{\iso}(\Omega_j),
% \end{equation}
% where the supremum is taken among all exhaustions $(\Omega_j)_{j\in \N}$. 
% \end{definition}
% It is immediately clear that such a concept of mass is well defined, and does not need any asymptotic assumption on the underlying metric.
% It is natural to wonder if this mass satisfies the Riemannian Penrose Inequality. The answer is known to be positive when the manifold $(M,g)$ satisfies strong asymptotic assumption, as \cite{jauregui_lower_2021} proved its equivalence with the $\ADM$ mass, following and strengthening the original argument of Huisken \cite{huisken_isoperimetric_2006}. 

% In this paper, we positively answer this question in the great generality of strongly $1$-nonparabolic spaces. With this locution, inspired by and coherent with \cite{ni_mean_2007}, we mean that for every $\Omega\subset M$ homologous to $\partial M$ with smooth boundary, there exists a solution $w_1\in \Lip_{\loc}(M\smallsetminus \Int \Omega)$ weakly solving the weak IMCF problem
% \begin{equation}\label{eq:IMCF}
%  \begin{cases}
%  \div\left( \frac{ \D w_1}{\abs{\D w_1}}\right) &=& \abs{ \D w_1} & \text{on $M\smallsetminus \Omega$,}\\
%  w_1 &=& 0 & \text{on $\partial \Omega$,}\\
%  w_1 &\to& +\infty & \text{as $\dist(x,o) \to +\infty$}.
%  \end{cases}
% \end{equation} 
% The following is the Riemannian Penrose Inequality for the Isoperimetric mass together with its rigidity statement.

% \begin{theorem}[Isoperimetric Riemannian Penrose Inequality]
% \label{thm:isoperimetric_penrose_intro}
% Let $(M,g)$ be a complete, strongly $1$-nonparabolic Riemannian $3$-manifold with nonnegative scalar curvature and with smooth, compact, minimal and minimising (possibly empty) boundary. Assume that $H_2(M, \partial M; \Z)=\set{0}$. For every $\Sigma $ connected component of $\partial M$ it holds
% \begin{equation}\label{eq:isoperimetric_penrose}
%  \sqrt{\frac{ \abs{\Sigma}}{16 \pi}} \leq \ma_{\iso}.
% \end{equation}
% Moreover, the equality holds in \cref{eq:isoperimetric_penrose} if and only if $(M,g)$ is isometric to the Schwarzschild manifold
% \begin{equation}
%  \left(\R^n\smallsetminus \set{ \abs{x} < 2 \ma_{\iso}}, \left( 1+ \frac{ \ma_{\iso}}{2 \abs{x}}\right)^4(\eum_{ij}\dd x^i \otimes \dd x^j)\right).
% \end{equation}
% \end{theorem}

% The condition $H_2(M, \partial M; \Z)=\set{0}$ ensures that the level sets of $w_1$ remain connected once they start at a subset with connected boundary. We stress the fact that we are not requiring any specific asymptotic assumption on the metric but the existence of the weak IMCF (possibly with jumps as in \cite{huisken_inverse_2001}). This condition is satisfied for example on manifolds with lower Ricci bounds and such that an Euclidean-like Isoperimetric inequality holds \cite[Theorem 1.7]{mari_flow_2022}, or whenever there exists a subsolution to \cref{eq:IMCF} starting at some bounded subset \cite[Weak Existence Theorem 3.1]{huisken_inverse_2001}. The proof of \cref{thm:isoperimetric_penrose_intro} combines the monotonicity of 
% the \emph{Hawking mass}
% \begin{equation}
%  \ma_{H}(\partial \Omega)= \frac{ \abs{ \partial \Omega_t}^{\frac{1}{2}}}{16 \pi^{\frac{3}{2}}} \left( 4 \pi - \int_{\partial \Omega}\frac{\H^2}{4} \dif \sigma \right)
% \end{equation}
% along the level sets $\partial \Omega_t =\partial \set{w_1 \leq t}$ of the weak IMCF \cite[Geroch Monotonicity Formula 5.8]{huisken_inverse_2001} with a novel, fairly simple, asymptotic comparison between $\ma_H(\partial\Omega_t)$ and $\ma_{\mathrm{iso}}(\Omega_t)$ as $t\to +\infty$ (see \cref{thm:mass_control_IMCF}). 

% \smallskip

% \cref{thm:isoperimetric_penrose_intro} provides new information also in the basic situation of manifolds that are $\CS^0$-asymptototic to a Schwarzschild space of nonnegative mass $\ma$. Indeed, we show that such parameter satisfies the expected Penrose Inequality and that it coincides in fact with the Isoperimetric mass, see \cref{thm:asysvarchild}. We emphasise that in this setting the classical notion of $\ADM$ mass is not even clearly defined, as it involves the asymptotic behaviour of derivatives of the metric.

% \begin{theorem}[Penrose Inequality in $\CS^0$-Asymptotically Schwarzschildian manifolds]
% \label{thm:asysvarchild}
% Let $(M, g)$ be a $\CS^0_\tau$-Asymptotically Schwarzschildian Riemannian $3$-manifold of mass $\ma \geq 0$. Assume that $g$ is a metric of nonnegative scalar curvature and that $\partial M$ is minimal and outward minimising. Assume also that $H_2(M, \partial M; \Z) = \set{0}$. Then, for every $\Sigma$ connected component of $\partial M$ the following Riemannian Penrose Inequality holds in terms of $\ma$
%  \begin{equation}
%  \label{eq:penrose-svarchild}
%  \sqrt{\frac{\abs{\Sigma}}{16 \pi}}\leq \ma,
% \end{equation}
% with equality achieved only in the Schwarzschild manifold of mass $\ma$. 

% Moreover, we have
% \begin{equation}
% \label{eq:identity-massiso} 
% \ma = \ma_{\iso}. 
% \end{equation}
% \end{theorem}

% \bigskip

% A more delicate argument provides the sharp Penrose Inequality for the classical $\ADM$ mass under the optimal $\CS^1_\tau$ asymptotic flatness, $\tau > 1/2,$ assumption, as well as the identification of such mass with the Isoperimetric one. 
% \begin{theorem}[Riemannian Penrose Inequality for the $\mathrm{ADM}$ mass]\label{thm:penrose_adm_intro}
% Let $(M,g)$ be a complete $\CS^{1}_{\tau}$-Asymptotically Flat Riemannian $3$-manifold, $\tau >1/2$, with nonnegative scalar curvature and smooth, compact, minimal and outward minimising (possibly empty) boundary. Assume that $H_2( M, \partial M; \Z)=\set{0}$. Then, for every $\Sigma $ connected component of $\partial M$ it holds
% \begin{equation}\label{eq:adm_penrose}
%  \sqrt{\frac{ \abs{\Sigma}}{16 \pi}} \leq \ma_{\ADM},
% \end{equation}
% with equality achieved if and only if $(M,g)$ is isometric to the Schwarzschild manifold
% \begin{equation}
%  \left(\R^n\smallsetminus \set{ \abs{x} < 2 \ma_{\ADM}}, \left( 1+ \frac{ \ma_{\ADM}}{2 \abs{x}}\right)^4(\eum_{ij} \dd x^i \otimes \dd x^j)\right).
% \end{equation}

% Moreover, we have
% \begin{equation}
% \label{eq:idadm}
%  \ma_{\iso}=\ma_{\ADM}.
% \end{equation}
% \end{theorem}
% Huisken-Ilmanen's proof through weak IMCF, and similarly the very recent \cite{agostiniani_riemannian_2022} through $p$-harmonic potentials, require the faster $\CS^1_1$--asymptotic flatness coupled with an asymptotically quadratically nonnegative Ricci curvature assumption. On the other hand, Bray's stronger version of the Penrose inequality \cite{bray_proof_2001}, in force for possibly disconnected horizons, is proved requiring $\CS^{2}_\tau$--asymptotic flatness. Asymptotic conditions on second derivatives of the metric are in fact commonly assumed even for proving the weaker Positive Mass Theorem along the nowadays classical arguments of Schoen-Yau \cite{schoen_proof_1979, schoen_proof_1981} and Witten \cite{witten_1981, parker-taubes}, or through the recent new proofs of \cite{bray-karazas-khuri-stern} and of \cite{agostiniani_green_2021}. In particular, to the best of our knowledge, not even a Positive Mass Theorem was known yet, under the above optimal decay assumptions. 

% \smallskip

% \textcolor{blue}{Our proof of \cref{thm:penrose_adm_intro} combines Huisken-Ilmanen's monotonicity of the Hawking mass along the weak IMCF with the monotonicity of the \emph{$2$-Hawking mass}
% \begin{equation}
% \label{eq:2hawking}
%  \ma^{\tph}_{H}(\partial \Omega) = \frac{\ncapa_2(\partial \Omega)}{8 \pi}\left[4\pi + \int_{\partial \Omega}{\abs{\D w_2}^2}\dif \sigma - \int_{\partial \Omega}{\abs{ \D w_2} }\H \dif \sigma \right]
% \end{equation}
% along the level sets of $w_2 = -\log u$, where $u$ the harmonic potential of the initial set. Such monotonicity was discovered in \cite{agostiniani_green_2021}. More precisely, we are exploiting the linear nature of the latter level set flow to obtain a reinforced asymptotic knowledge of the quantities involved in \cref{eq:2hawking}. This knowledge is sufficient to bound $\ma^{\tph}_{H}(\partial \Omega_t)$ from above in terms of $\ma_{\ADM}$ (see \cref{thm:bound_2_hawking}) and in turn yields a uniform (nonsharp) bound for the Hawking mass of any initial set. 
% We implement this a priori bound in the asymptotic argument which leads to \cref{thm:isoperimetric_penrose_intro}, obtaining an improved asymptotic behaviour of the mean curvature along the weak IMCF. Coupling it with the final analysis in the proof of \cite[Asymptotic Comparison Lemma 7.4]{huisken_inverse_2001}, we sharply control the Hawking mass of a relevant class of subsets $\Omega \subseteq M$ by the $\ADM$ mass
% \begin{equation}\label{eq:hawking_madm_intro}
%  \ma_{\H}(\partial \Omega) \leq \ma_{\ADM}.
% \end{equation}
% This inequality, applied to $\partial \Omega = \Sigma$, implies at once the \cref{eq:adm_penrose} Penrose inequality.
% The identity \cref{eq:idadm}, as well as \cref{eq:identity-massiso}, is deduced substantially combining \cref{eq:hawking_madm_intro} with the main result of \cite{jauregui_lower_2021} (see \cref{thm:bound_hawking_to_bound_iso} below) and with the limit behaviour of the quasi-local Isoperimetric masses of geodesic balls computed in \cite{fan_largesphere_2009}.
% }

% \textcolor{purple}{QUELLO CHE SEGUE E' IN ALTERNATIVA ALLA PORZIONE BLU.}

% Our proof of \cref{thm:penrose_adm_intro} combines Huisken-Ilmanen's monotonicity of the Hawking mass along the weak IMCF with the monotonicity of the \emph{$2$-Hawking mass}
% \begin{equation}
% \label{eq:2hawking}
%  \ma^{\tph}_{H}(\partial \Omega) = \frac{\ncapa_2(\partial \Omega)}{8 \pi}\left[4\pi + \int_{\partial \Omega}{\abs{\D w_2}^2}\dif \sigma - \int_{\partial \Omega}{\abs{ \D w_2} }\H \dif \sigma \right]
% \end{equation}
% along the level sets of $w_2 = -\log u$, where $u$ the harmonic potential of the initial set. Such monotonicity was discovered in \cite{agostiniani_green_2021}. More precisely, we are exploiting the linear nature of the latter level set flow in order to bound $\ma^{\tph}_{H}(\partial \Omega_t)$ from above in terms of $\ma_{\ADM}$ (see \cref{thm:bound_2_hawking}). This in turn yields a uniform bound for the Hawking mass of any initial set. We are then exploiting this a priori (nonsharp) bound, coupled with suitable refinements of the asymptotic argument that lead to \cref{thm:isoperimetric_penrose_intro}, to sharply control the limit of $\ma(\partial \Omega_t)$ as $t \to \infty$ by the $\mathrm{ADM}$ mass. 
% In particular, we take advantage of the specifically crafted quantity
% \begin{equation}
% \label{eq:minkintro}
%  \ma_{M}(\partial \Omega_t) = \frac{\sqrt{\abs{\partial \Omega_t}}}{16 \pi } \left( 4 \sqrt{\pi} - \frac{1}{\sqrt{\abs{ \partial \Omega}}} \int_{\partial \Omega_t}\kern-.1cm\H \dif \sigma\right)
% \end{equation}
% defined along the IMCF. We refer to it as \emph{Minkowski mass}. Its main feature is that of being asymptotically encapsulated between the Hawking and the quasi-local isoperimetric mass of $\Omega_t$; this will in turn result in some key asymptotic information about the $L^2$--convergence of the second fundamental forms and of the mean curvatures of the level sets along the flow.
% We will finally be able to conclude the analysis of the Hawking mass with the sharp bound 
% \begin{equation}
% \label{eq:boundhwakingintro}
%  \ma_{H}(\partial \Omega) \leq \lim_{t \to +\infty} \ma_{H}(\partial \Omega_t) \leq \ma_{\mathrm{ADM}},
% \end{equation}
% and obtain the claimed Penrose inequality.

% The identity \cref{eq:idadm}, and similarly \cref{eq:identity-massiso}, is deduced substantially combining \cref{eq:boundhwakingintro} with the main result of \cite{jauregui_lower_2021}, see \cref{thm:bound_hawking_to_bound_iso} below, and with the limit behaviour of the quasi local Isoperimetric masses of geodesic balls computed in \cite{fan_largesphere_2009}. 


